ReconVAT: A Semi-Supervised Automatic Music Transcription Framework for Low-Resource Real-World Data

Most of the current supervised automatic music transcription (AMT) models lack the ability to generalize. This means that they have trouble transcribing real-world music recordings from diverse musical genres that are not presented in the labelled training data. In this paper, we propose a semi-supervised framework, ReconVAT, which solves this issue by leveraging the huge amount of available unlabelled music recordings. The proposed ReconVAT uses reconstruction loss and virtual adversarial training. When combined with existing U-net models for AMT, ReconVAT achieves competitive results on common benchmark datasets such as MAPS and MusicNet. For example, in the few-shot setting for the string part version of MusicNet, ReconVAT achieves F1-scores of 61.0% and 41.6% for the note-wise and note-with-offset-wise metrics respectively, which translates into an improvement of 22.2% and 62.5% compared to the supervised baseline model. Our proposed framework also demonstrates the potential of continual learning on new data, which could be useful in real-world applications whereby new data is constantly available.

==> Tables/full_MAPS.tex <==
% \begin{table*}[h]
% \centering
%  \caption{Transcription accuracy in terms of different metrics and its respective precision (P), recall (R) and F1-score (F1) when training on the full version of the MAPS dataset. The baseline models are highlighted in grey.}
% \small
% \resizebox{\textwidth}{!}
% {\begin{tabular}{l|ccc|ccc|ccc|}
% \cline{2-10}
% \multicolumn{1}{c|}{}                             & \multicolumn{3}{c|}{\textbf{Frame}} & \multicolumn{3}{c|}{\textbf{Note}}            & \multicolumn{3}{c|}{\textbf{Note w/ offset}}  \\ \cline{2-10} 
% \multicolumn{1}{c|}{}                             & P              & R    & F1          & P             & R             & F1            & P             & R             & F1            \\ \hline
% \multicolumn{1}{|l|}{U-net VAT} & 86.6 ± 5.4& 71.5 ± 9.4& 77.9 ± 6.7& 64.5 ± 13.2& 64.2 ± 12.6& 64.0 ± 12.3& 40.8 ± 11.6& 40.9 ± 12.1& 40.6 ± 11.5 \\ \hline
% \multicolumn{1}{|l|}{U-net-R VAT} & 88.8 ± 6.0& 72.7 ± 9.0& 79.5 ± 6.5& 74.0 ± 9.3& 63.3 ± 13.3& 67.9 ± 11.2& 49.7 ± 10.1& 42.9 ± 12.5& 45.8 ± 11.3 \\ \hline
% \rowcolor{lightgray} 
% \multicolumn{1}{|l|}{U-net~\cite{cheukICPR}}   & 84.6 ± 6.0& 70.8 ± 8.9& 76.7 ± 6.5& 55.8 ± 12.6& 62.0 ± 11.9& 58.4 ± 11.7& 34.5 ± 11.3& 38.5 ± 12.0& 36.2 ± 11.4        \\ \hline
% \rowcolor{lightgray} 
% \multicolumn{1}{|l|}{U-net-R~\cite{cheukICPR}} & 86.2 ± 6.2& 72.7 ± 10.0& 78.4 ± 7.0& 68.5 ± 10.5& 61.0 ± 13.1& 64.2 ± 11.4& 45.5 ± 11.1& 40.8 ± 12.9& 42.8 ± 11.9 \\ \hline
% \multicolumn{1}{|l|}{U-net-O} & 89.6 ± 6.0& 58.8 ± 9.9& 70.4 ± 7.5& 85.8 ± 7.8& 66.3 ± 11.0& 74.5 ± 9.2& 53.1 ± 9.5& 41.5 ± 11.3& 46.4 ± 10.6 \\ \hline
% \multicolumn{1}{|l|}{U-net-O VAT} & 90.9 ± 6.1& 60.5 ± 9.5& 72.2 ± 7.5& 89.8 ± 8.3& 65.0 ± 11.1& 75.1 ± 9.5& 58.7 ± 9.9& 42.9 ± 11.3& 49.4 ± 10.8 \\ \hline
% \multicolumn{1}{|l|}{U-net-RO} & 89.9 ± 6.6& 60.4 ± 10.8& 71.6 ± 8.3& 86.1 ± 7.9& 67.3 ± 11.2& 75.2 ± 9.2& 52.8 ± 10.1& 41.7 ± 11.6& 46.4 ± 10.9 \\ \hline
% \multicolumn{1}{|l|}{U-net-RO VAT} & 85.9 ± 7.2& 72.0 ± 8.7& 77.9 ± 6.5& 80.9 ± 7.0& 70.6 ± 11.2& 75.1 ± 8.6& 54.3 ± 9.8& 47.6 ± 11.8& 50.5 ± 10.6 \\ \hline
% \rowcolor{lightgray} 
% \multicolumn{1}{|l|}{O\&F~\cite{Hawthorne2017OnsetsAF} } & 89.3 ± 6.4& 65.6 ± 9.7& 75.2 ± 7.3& 85.2 ± 7.8& 73.3 ± 11.4& 78.6 ± 9.3& 53.8 ± 9.8& 46.7 ± 12.0& 49.8 ± 10.9  \\ \hline

% % \rowcolor{lightgray} 
% % \multicolumn{1}{|l|}{Tensorflow version~\cite{Hawthorne2017OnsetsAF}} & 88.5             & 70.9    & 78.3       & 84.2             & 80.7             & 82.3          & 51.3             & 49.3             & 50.2          \\ \hline
% \end{tabular}}
% %  \vspace{-6pt}
%  \label{tab:full_MAPS}
% \end{table*}




\begin{table*}[h]
\centering
 \caption{Transcription accuracy (mean + STD) in terms of different metrics and their respective precision (P), recall (R), and F1-score (F1) when training on different variations of the MAPS dataset. The baseline and existing models are highlighted in grey.}
\small
\resizebox{\textwidth}{!}
{\begin{tabular}{ll|ccc|ccc|ccc|}
\cline{3-11}
\multicolumn{1}{c}{}  &\multicolumn{1}{c|}{}                             & \multicolumn{3}{c|}{\textbf{Frame}} & \multicolumn{3}{c|}{\textbf{Note}}            & \multicolumn{3}{c|}{\textbf{Note w/ offset}}  \\ \cline{3-11} 
&\multicolumn{1}{c|}{\textbf{Full}}                           & P              & R    & F1          & P             & R             & F1            & P             & R             & F1            \\ \cline{2-11}
A1&\multicolumn{1}{|l|}{U-net VAT} & 86.6 ± 5.4& 71.5 ± 9.4& 77.9 ± 6.7& 64.5 ± 13.2& 64.2 ± 12.6& 64.0 ± 12.3& 40.8 ± 11.6& 40.9 ± 12.1& 40.6 ± 11.5 \\ \cline{2-11} 
A2&\multicolumn{1}{|l|}{U-net-R VAT} & 88.8 ± 6.0& \textbf{72.7 ± 9.0}& \textbf{79.5 ± 6.5}& 74.0 ± 9.3& 63.3 ± 13.3& 67.9 ± 11.2& 49.7 ± 10.1& 42.9 ± 12.5& 45.8 ± 11.3 \\ \cline{2-11}
A3&\multicolumn{1}{|l|}{U-net~\cite{cheukICPR}}   & 84.6 ± 6.0& 70.8 ± 8.9& 76.7 ± 6.5& 55.8 ± 12.6& 62.0 ± 11.9& 58.4 ± 11.7& 34.5 ± 11.3& 38.5 ± 12.0& 36.2 ± 11.4        \\ \cline{2-11} 
A4&\multicolumn{1}{|l|}{U-net-R~\cite{cheukICPR}} & 86.2 ± 6.2& 72.7 ± 10.0& 78.4 ± 7.0& 68.5 ± 10.5& 61.0 ± 13.1& 64.2 ± 11.4& 45.5 ± 11.1& 40.8 ± 12.9& 42.8 ± 11.9 \\ \cline{2-11} 
A5&\multicolumn{1}{|l|}{U-net-O} & 89.6 ± 6.0& 58.8 ± 9.9& 70.4 ± 7.5& 85.8 ± 7.8& 66.3 ± 11.0& 74.5 ± 9.2& 53.1 ± 9.5& 41.5 ± 11.3& 46.4 ± 10.6 \\ \cline{2-11} 
A6&\multicolumn{1}{|l|}{U-net-O VAT} &\textbf{ 90.9 ± 6.1}& 60.5 ± 9.5& 72.2 ± 7.5& \textbf{89.8 ± 8.3}& 65.0 ± 11.1& 75.1 ± 9.5& \textbf{58.7 ± 9.9} & 42.9 ± 11.3& 49.4 ± 10.8 \\ \cline{2-11} 
A7&\multicolumn{1}{|l|}{U-net-RO} & 89.9 ± 6.6& 60.4 ± 10.8& 71.6 ± 8.3& 86.1 ± 7.9& 67.3 ± 11.2& 75.2 ± 9.2& 52.8 ± 10.1& 41.7 ± 11.6& 46.4 ± 10.9 \\ \cline{2-11} 
A8&\multicolumn{1}{|l|}{U-net-RO VAT} & 85.9 ± 7.2& 72.0 ± 8.7& 77.9 ± 6.5& 80.9 ± 7.0& 70.6 ± 11.2& 75.1 ± 8.6& 54.3 ± 9.8& \textbf{47.6 ± 11.8}& \textbf{50.5 ± 10.6} \\ \cline{2-11} 
A9&\multicolumn{1}{|l|}{O\&F~\cite{Hawthorne2017OnsetsAF} } & 89.3 ± 6.4& 65.6 ± 9.7& 75.2 ± 7.3& 85.2 ± 7.8& \textbf{73.3 ± 11.4}& \textbf{78.6 ± 9.3}& 53.8 ± 9.8& 46.7 ± 12.0& 49.8 ± 10.9  \\ \cline{2-11} 

&\multicolumn{1}{c|}{\textbf{Small}}& P& R& F1& P& R& F1& P& R& F1 \\ \cline{2-11}      
B1&\multicolumn{1}{|l|}{U-net VAT} & 79.1 ± 6.6& 56.9 ± 11.7& 65.4 ± 8.7& 52.4 ± 11.9& 60.1 ± 12.6& 55.5 ± 11.3& 26.2 ± 9.8& 30.3 ± 11.6& 27.8 ± 10.3 \\ \cline{2-11} 
B2&\multicolumn{1}{|l|}{U-net-R VAT} & 79.7 ± 6.1& 59.9 ± 11.0& 67.7 ± 7.8& 57.2 ± 11.9& 61.0 ± 12.0& 58.6 ± 11.1& 29.2 ± 10.3& 31.3 ± 11.3& 30.0 ± 10.5 \\ \cline{2-11} 
B3&\multicolumn{1}{|l|}{U-net~\cite{cheukICPR}}   & 75.4 ± 6.6& 57.1 ± 9.6& 64.5 ± 7.3& 35.4 ± 8.3& 57.5 ± 11.6& 43.5 ± 8.9& 17.0 ± 6.9& 27.6 ± 10.6& 20.9 ± 8.0       \\ \cline{2-11} 
B4&\multicolumn{1}{|l|}{U-net-R~\cite{cheukICPR}} & 81.2 ± 6.1& \textbf{61.1 ± 11.1}& \textbf{69.1 ± 8.1}& 51.0 ± 10.3& \textbf{61.3 ± 12.4}& 55.3 ± 10.6& 26.2 ± 9.8& \textbf{31.8 ± 12.4}& 28.6 ± 10.7 \\ \cline{2-11} 
B5&\multicolumn{1}{|l|}{U-net-O} & 88.3 ± 6.3& 38.4 ± 10.2& 52.6 ± 9.8& 81.9 ± 7.9& 50.1 ± 11.3& 61.6 ± 9.8& 41.0 ± 10.1& 25.6 ± 10.1& 31.2 ± 10.2 \\ \cline{2-11} 
B6&\multicolumn{1}{|l|}{U-net-O VAT} & 89.5 ± 6.6& 41.0 ± 10.5& 55.4 ± 10.0& \textbf{86.8 ± 8.8}& 52.3 ± 12.1& 64.7 ± 10.7& 44.0 ± 10.8& 27.0 ± 10.4& 33.1 ± 10.7 \\ \cline{2-11} 
B7&\multicolumn{1}{|l|}{U-net-RO} & 88.0 ± 6.3& 44.9 ± 11.2& 58.5 ± 10.1& 83.4 ± 8.7& 55.8 ± 12.2& 66.3 ± 10.3& 42.8 ± 10.3& 29.2 ± 10.7& 34.4 ± 10.6 \\ \cline{2-11} 
B8&\multicolumn{1}{|l|}{U-net-RO VAT} & \textbf{90.0 ± 6.2}& 43.9 ± 10.6& 58.2 ± 9.7& 86.2 ± 8.6& 57.1 ± 11.5& \textbf{68.2 ± 10.0}& \textbf{44.6 ± 11.7}& 30.0 ± 11.0& \textbf{35.6 ± 11.3 }\\ \cline{2-11} 
B9&\multicolumn{1}{|l|}{O\&F~\cite{Hawthorne2017OnsetsAF}} & 89.7 ± 5.8& 37.7 ± 10.4& 52.2 ± 10.4& 85.3 ± 8.6& 51.2 ± 13.1& 63.1 ± 11.4& 41.8 ± 10.5& 25.5 ± 10.2& 31.2 ± 10.4  \\ \cline{2-11} 

&\multicolumn{1}{c|}{\textbf{One-shot}} & P& R& F1          & P             & R             & F1            & P             & R             & F1            \\ \cline{2-11} 
C1&\multicolumn{1}{|l|}{U-net VAT}                & 75.6 ± 6.6& \textbf{46.1 ± 11.1}& \textbf{56.2 ± 9.0}& 42.7 ± 11.0& 55.2 ± 12.7& 47.1 ± 9.6& 17.1 ± 7.8& 22.1 ± 9.7& 18.9 ± 8.1 \\ \cline{2-11} 
C2&\multicolumn{1}{|l|}{U-net-R VAT}              & 71.6 ± 6.0& 43.6 ± 9.5& 53.3 ± 7.3& 36.4 ± 8.5& \textbf{61.5 ± 12.0}& 45.2 ± 8.5& 13.6 ± 6.6& \textbf{22.8 ± 10.4}& 16.8 ± 7.7 \\ \cline{2-11} 
C3&\multicolumn{1}{|l|}{U-net~\cite{cheukICPR}}   & 61.9 ± 5.8& 41.8 ± 9.1& 49.2 ± 6.9& 24.7 ± 7.6& 49.6 ± 10.6& 32.2 ± 7.9& 8.8 ± 5.6& 17.0 ± 8.5& 11.3 ± 6.5        \\ \cline{2-11} 
C4&\multicolumn{1}{|l|}{U-net-R~\cite{cheukICPR}} & 74.8 ± 5.9& 41.2 ± 10.4& 52.2 ± 8.5  &    33.6 ± 9.4& 54.5 ± 11.5& 40.7 ± 8.8   & 12.5 ± 7.2& 19.8 ± 10.0& 15.0 ± 8.1 \\ \cline{2-11} 
C5&\multicolumn{1}{|l|}{U-net-O}                  & 87.7 ± 7.2& 17.4 ± 7.0 & 28.4 ± 9.3  &    \textbf{85.7 ± 6.6}& 27.7 ± 10.0& 40.9 ± 11.3  & \textbf{34.5 ± 10.6}& 11.4 ± 6.1& 16.8 ± 7.7 \\ \cline{2-11} 
C6&\multicolumn{1}{|l|}{U-net-O VAT}              & 72.9 ± 9.4& 22.9 ± 8.8 & 33.5 ± 9.1  &    57.9 ± 10.2& 43.6 ± 12.4& 47.9 ± 7.6  & 17.1 ± 7.8& 13.0 ± 7.0& 14.2 ± 6.8 \\ \cline{2-11} 
C7&\multicolumn{1}{|l|}{U-net-RO}                 & 87.7 ± 7.5& 21.4 ± 9.0& 33.4 ± 11.1  & 82.0 ± 7.1& 33.4 ± 11.7& 46.3 ± 11.9& 34.4 ± 10.0& 14.6 ± 7.9& 20.0 ± 9.0 \\ \cline{2-11} 
C8&\multicolumn{1}{|l|}{U-net-RO VAT} & 86.1 ± 6.8& 31.4 ± 9.8& 45.0 ± 10.3& 77.2 ± 9.8& 51.5 ± 12.4& \textbf{60.7 ± 9.6}& 31.4 ± 10.4& 21.1 ± 9.1& \textbf{24.8 ± 9.2} \\ \cline{2-11} 
C9&\multicolumn{1}{|l|}{O\&F~\cite{Hawthorne2017OnsetsAF}}     & \textbf{88.0 ± 6.8}& 12.4 ± 4.8& 21.3 ± 7.2& 83.5 ± 8.2& 30.5 ± 10.4& 43.7 ± 11.2& 23.1 ± 11.4& 8.3 ± 4.7& 11.9 ± 6.3  \\ \cline{2-11} 

\end{tabular}}
 \label{tab:full_MAPS}
\end{table*}



==> Tables/string_MusicNet.tex <==
\begin{table*}[h]
\centering
 \caption{Transcription accuracy (mean + standard deviation) in terms of different metrics and their respective precision (P), recall (R), and F1-score (F1) when training on the different variations of the MusicNet dataset. The baseline and existing models are highlighted in grey.}
\small 
\resizebox{\textwidth}{!}
{\begin{tabular}{ll|ccc|ccc|ccc|}
\cline{3-11}
&\multicolumn{1}{c|}{}                             & \multicolumn{3}{c|}{\textbf{Frame}} & \multicolumn{3}{c|}{\textbf{Note}}            & \multicolumn{3}{c|}{\textbf{Note w/ offset}}  \\ \cline{3-11} 
&\multicolumn{1}{c|}{\textbf{Strings}}                             & P              & R    & F1          & P             & R             & F1            & P             & R             & F1            \\ \cline{2-11}
D1&\multicolumn{1}{|l|}{U-net VAT} & 76.1 ± 7.2& 52.4 ± 11.9& 61.7 ± 10.2& 58.1 ± 13.9& 51.2 ± 15.1& 54.2 ± 14.3& 39.6 ± 17.8& 35.4 ± 18.4& 37.2 ± 18.1 \\ \cline{2-11}
D2&\multicolumn{1}{|l|}{U-net-R VAT} &\textbf{ 78.9 ± 4.8}& 60.7 ± 9.8& \textbf{68.4 ± 7.7}& 63.6 ± 13.8& \textbf{58.8 ± 14.3}& \textbf{61.0 ± 13.8}& 43.3 ± 18.8& 40.2 ± 18.9& \textbf{41.6 ± 18.7} \\ \cline{2-11}
\rowcolor{lightgray} 
D3&\multicolumn{1}{|l|}{U-net~\cite{cheukICPR}}   & 67.1 ± 6.9& 50.7 ± 12.9& 57.4 ± 10.5& 41.8 ± 12.5& 46.1 ± 12.7& 43.7 ± 12.5& 24.6 ± 13.4& 26.7 ± 14.0& 25.6 ± 13.7        \\ \cline{2-11}
\rowcolor{lightgray} 
D4&\multicolumn{1}{|l|}{U-net-R~\cite{cheukICPR}} & 71.7 ± 2.9& \textbf{62.8 ± 10.6}& 66.6 ± 6.9& 53.1 ± 10.7& 57.4 ± 11.9& 55.1 ± 11.1& 37.6 ± 14.1& \textbf{40.9 ± 16.4}& 39.1 ± 15.2 \\ \cline{2-11}
\rowcolor{lightgray} 
D5&\multicolumn{1}{|l|}{Multi-Inst~\cite{MultiInstrument}} & 71.4 ± 6.2& 59.5 ± 13.1& 64.5 ± 9.6& 56.5 ± 16.7& 45.1 ± 18.4& 49.9 ± 17.8& 33.7 ± 19.3& 27.8 ± 18.4& 30.3 ± 18.9 \\ \cline{2-11}
D6&\multicolumn{1}{|l|}{U-net-O} & 70.0 ± 8.4& 25.3 ± 13.4& 35.7 ± 13.8& 59.9 ± 10.7& 24.6 ± 13.0& 33.9 ± 13.6& 35.4 ± 11.3& 15.0 ± 9.9& 20.5 ± 11.0 \\ \cline{2-11}
D7&\multicolumn{1}{|l|}{U-net-O VAT} & 65.2 ± 18.9& 27.6 ± 13.5& 38.2 ± 15.6& 52.7 ± 14.2& 27.8 ± 14.5& 35.7 ± 14.9& 31.5 ± 13.4& 17.4 ± 12.6& 22.0 ± 13.5 \\ \cline{2-11}
D8&\multicolumn{1}{|l|}{U-net-RO} & 79.1 ± 1.1& 39.3 ± 18.7& 50.1 ± 16.6& 68.5 ± 12.3& 39.4 ± 17.2& 48.6 ± 16.1& 49.0 ± 17.1& 29.9 ± 17.8& 36.3 ± 18.5 \\ \cline{2-11}
D9&\multicolumn{1}{|l|}{U-net-RO VAT} & 78.0 ± 4.0& 36.9 ± 10.5& 49.5 ± 10.1& \textbf{69.6 ± 13.7}& 37.6 ± 11.4& 48.4 ± 11.9& \textbf{50.1 ± 18.3}& 27.8 ± 13.4& 35.4 ± 15.4 \\ \cline{2-11}
\rowcolor{lightgray} 
D10&\multicolumn{1}{|l|}{O\&F~\cite{Hawthorne2017OnsetsAF}} & 75.3 ± 3.1& 22.5 ± 12.0& 33.1 ± 14.6& 69.0 ± 15.8& 22.6 ± 12.1& 32.9 ± 14.8& 41.7 ± 18.2& 15.3 ± 11.2& 21.7 ± 14.5  \\ \cline{2-11}

&\multicolumn{1}{c|}{\textbf{Woodwinds}}                             & P              & R    & F1          & P             & R             & F1            & P             & R             & F1            \\ \cline{2-11}
E1&\multicolumn{1}{|l|}{U-net VAT} & 69.0 ± 9.6& 62.4 ± 1.2& 65.1 ± 3.7& 44.4 ± 3.1& 40.5 ± 2.5& 42.2 ± 0.0& 16.1 ± 1.6& 14.6 ± 0.5& 15.3 ± 0.5 \\ \cline{2-11}
E2&\multicolumn{1}{|l|}{U-net-R VAT} &\textbf{ 69.8 ± 8.3}& 65.8 ± 2.0& 67.4 ± 2.8& \textbf{48.6 ± 3.5}& 47.9 ± 1.1& \textbf{48.2 ± 1.2}& \textbf{22.1 ± 3.1}& \textbf{21.7 ± 1.0}& \textbf{21.8 ± 2.0} \\ \cline{2-11}
\rowcolor{lightgray} 
E3&\multicolumn{1}{|l|}{U-net~\cite{cheukICPR}}  & 62.6 ± 9.6& 65.7 ± 2.9& 63.5 ± 3.7& 33.6 ± 2.4& 39.9 ± 1.1& 36.4 ± 1.0& 11.6 ± 1.4& 13.7 ± 0.3& 12.5 ± 0.9        \\ \cline{2-11}
\rowcolor{lightgray} 
E4&\multicolumn{1}{|l|}{U-net-R~\cite{cheukICPR}} & 65.4 ± 6.7& 71.4 ± 4.3& \textbf{67.8 ± 1.7}& 40.5 ± 5.8& \textbf{52.5 ± 0.6}& 45.4 ± 3.5& 16.9 ± 5.2& 21.3 ± 3.5& 18.7 ± 4.7 \\ \cline{2-11}
\rowcolor{lightgray} 
E5&\multicolumn{1}{|l|}{Multi-Inst~\cite{MultiInstrument}} & 64.4 ± 9.4&\textbf{ 71.8 ± 2.7}& 67.3 ± 4.1& 43.5 ± 2.8& 33.6 ± 0.6& 37.9 ± 0.7& 17.1 ± 2.5& 13.2 ± 0.9& 14.9 ± 1.5 \\ \cline{2-11}

% \rowcolor{lightgray} 
% \multicolumn{1}{|l|}{Tensorflow version~\cite{Hawthorne2017OnsetsAF}} & 88.5             & 70.9    & 78.3       & 84.2             & 80.7             & 82.3          & 51.3             & 49.3             & 50.2          \\ \cline{2-11}
\end{tabular}}
%  \vspace{-6pt}
 \label{tab:string_MusicNet}
\end{table*}

==> Tables/string_data.tex <==
\begin{table*}[hbt!]
  \caption{The training and test split for the string version of MusicNet.}
  \label{tab:string_data}
  \begin{tabular}{P{3cm}P{1.5cm}P{7.2cm}P{1.5cm}}
    \toprule
    Genre & Labelled Train ID & Unlabelled Train ID & Test ID\\
    \midrule
    Solo violin & 2186 & 2241, 2242, 2243, 2244, 2288, 2289, 2659 & 2191\\\hline
    Violin and harpsichord & 2282 & 2283, 2284, 2285 & N.A.\\\hline
    Accompanied violin & 2330 & 2334, 2335, 2336, 2341, 2342, 2397, 2398, 2420, 2462, 2463, 2466,
      2501, 2502, 2570, 2571, 2572, 2573, 2626, 2627, 2629 & 2628\\\hline
    String quartet & 1788 & 1789, 1790, 1791, 1792, 1793, 1805, 1807, 1822, 1824, 1835, 1859,
      1916, 1918, 1919, 1922, 1923, 1931, 1932, 1933, 2104, 2105, 2138,
      2140, 2177, 2178, 2179, 2180, 2313, 2314, 2315, 2365, 2366, 2368,
      2376, 2377, 2379, 2381, 2383, 2384, 2403, 2431, 2432, 2433, 2451,
      2480, 2481, 2482, 2483, 2494, 2497, 2560, 2562, 2621, 2622 & 2106\\\hline
    String sextet & 2147 & 2154, 2155, 2156, 2157 & N.A.\\\hline
    Viola Quintet & 1742 & N.A. & N.A.\\\hline
    Solo cello & 2217 & 2218, 2219, 2220, 2221, 2222, 2293, 2294, 2295, 2296, 2297 & 2298\\\hline
    Accompanied Cello & 2112 & 2113, 2114, 2521, 2522, 2523, 2586 & N.A.\\\hline
  \bottomrule
  Total number & 8 & 104 & 4
\end{tabular}
\end{table*}

==> Tables/woodwind_MusicNet.tex <==
\begin{table*}[h]
\centering
 \caption{Transcription accuracy in terms of different metrics and their respective precision (P), recall (R), and F1-score (F1) when training on the woodwind version of the MusicNet dataset. The baseline models are highlighted in grey.}
\small
\resizebox{\textwidth}{!}
{\begin{tabular}{l|ccc|ccc|ccc|}
\cline{2-10}
\multicolumn{1}{c|}{}                             & \multicolumn{3}{c|}{\textbf{Frame}} & \multicolumn{3}{c|}{\textbf{Note}}            & \multicolumn{3}{c|}{\textbf{Note w/ offset}}  \\ \cline{2-10} 
\multicolumn{1}{c|}{}                             & P              & R    & F1          & P             & R             & F1            & P             & R             & F1            \\ \hline
\multicolumn{1}{|l|}{U-net VAT} & 69.0 ± 9.6& 62.4 ± 1.2& 65.1 ± 3.7& 44.4 ± 3.1& 40.5 ± 2.5& 42.2 ± 0.0& 16.1 ± 1.6& 14.6 ± 0.5& 15.3 ± 0.5 \\ \hline
\multicolumn{1}{|l|}{U-net-R VAT} & 69.8 ± 8.3& 65.8 ± 2.0& 67.4 ± 2.8& 48.6 ± 3.5& 47.9 ± 1.1& 48.2 ± 1.2& 22.1 ± 3.1& 21.7 ± 1.0& 21.8 ± 2.0 \\ \hline
\rowcolor{lightgray} 
\multicolumn{1}{|l|}{U-net~\cite{cheukICPR}}  & 62.6 ± 9.6& 65.7 ± 2.9& 63.5 ± 3.7& 33.6 ± 2.4& 39.9 ± 1.1& 36.4 ± 1.0& 11.6 ± 1.4& 13.7 ± 0.3& 12.5 ± 0.9        \\ \hline
\rowcolor{lightgray} 
\multicolumn{1}{|l|}{U-net-R~\cite{cheukICPR}} & 65.4 ± 6.7& 71.4 ± 4.3& 67.8 ± 1.7& 40.5 ± 5.8& 52.5 ± 0.6& 45.4 ± 3.5& 16.9 ± 5.2& 21.3 ± 3.5& 18.7 ± 4.7 \\ \hline
\rowcolor{lightgray} 
\multicolumn{1}{|l|}{Multi-Inst~\cite{MultiInstrument}} & 64.4 ± 9.4& 71.8 ± 2.7& 67.3 ± 4.1& 43.5 ± 2.8& 33.6 ± 0.6& 37.9 ± 0.7& 17.1 ± 2.5& 13.2 ± 0.9& 14.9 ± 1.5 \\ \hline


% \rowcolor{lightgray} 
% \multicolumn{1}{|l|}{Tensorflow version~\cite{Hawthorne2017OnsetsAF}} & 88.5             & 70.9    & 78.3       & 84.2             & 80.7             & 82.3          & 51.3             & 49.3             & 50.2          \\ \hline
\end{tabular}}
%  \vspace{-6pt}
 \label{tab:woodwind_MusicNet}
\end{table*}

==> Tables/woodwind_data.tex <==
\begin{table*}[hbt!]
  \caption{The training and test split for the woodwind version of MusicNet.}
  \label{tab:woodwind_data}
  \begin{tabular}{P{3cm}P{1.5cm}P{7.2cm}P{1.5cm}}
    \toprule
    Genre & Labelled Train ID & Unlabelled Train ID & Test ID\\
    \midrule
    Accompanied Clarinet & 2116 & 2117, 2118, 2119 & N.A.\\\hline
    Clarinet Quintet & 1811 & 1812, 1813 & N.A.\\\hline
    Pairs Clarinet-Horn-Bassoon & 1817 & 1818, 2415, 2417 & 1819, 2416\\\hline
    Clarinet-Cello-Piano Trio & 2318 & 2319, 2320 & N.A.\\\hline
    Wind Octet & 2504 & 2505, 2506, 2507 & N.A.\\\hline
    Wind Quintet & 2075 & 2076, 2077, 2078, 2079, 2080, 2081, 2082, 2083 & N.A.\\\hline
  \bottomrule
  Total number & 6 & 21 & 2
\end{tabular}
\end{table*}
